Non-equilibrium critical behavior : An extended irreversible thermodynamics approach

Critical phenomena in non-equilibrium systems have been studied by means of a wide variety of theoretical and experimental approaches. Mode-coupling, renormalization group, complex Lie algebras and diagrammatic techniques are some of the usual theoretical tools. Experimental studies include light and inelastic neutron scattering, X-ray photon correlation spectroscopy, microwave interferometry and several other techniques. Nevertheless no conclusive reatment has been developed from the basic principles of a thermodynamic theory of irreversible processes. We have developed a formalism in which we obtain correlation functions as field averages of the associated functions. By applying such formalism we attempt to find out if the resulting correlation functions will inherit the mathematical properties (integrability, generalized homogeneity, scaling laws) of its parent potentials, and we will also use these correlation functions to study the behavior of macroscopic systems far from equilibrium, specially in the neighborhood of critical points or dynamic phase transitions. As a working example we will consider the mono-critical behavior of a non-equilibrium binary fluid mixture close to its consolute point.

==> tablitas.tex <==

\begin{table}[h!b!p!]
\caption{Table (default)}
\begin{tabular}{lll}
\hline
Alphabet Character & Vowel & Number \\
\hline
A & Yes & 1 \\
B & No & 2 \\
C & No & 3 \\
\hline
\end{tabular}
\label{table1}
\end{table} 
